Weighted-CEL0 sparse regularisation for molecule localisation in super-resolution microscopy with Poisson data

We propose a continuous non-convex variational model for Single Molecule Localisation Microscopy (SMLM) super-resolution in order to overcome light diffraction barriers. Namely, we consider a variation of the Continuous Exact $\ell_0$ (CEL0) penalty recently introduced to relax the $\ell_2-\ell_0$ problem where a weighted-$\ell_2$ data fidelity is considered to model signal-dependent Poisson noise. For the numerical solution of the associated minimisation problem, we consider an iterative reweighted $\ell_1$ (IRL1) strategy for which we detail efficient parameter computation strategies. We report qualitative and quantitative molecule localisation results showing that the proposed weighted-CEL0 (wCEL0) model improves the results obtained by CEL0 and state-of-the art deep-learning approaches for the high-density SMLM ISBI 2013 dataset.

==> ISBI/isbi_dataset.tex <==
The IEEE ISBI simulated dataset is a stack of $361$ images that represent 8 tubes of $30\ nm$ diameter.  The acquisitions are simulated with a size of $64\times 64$ pixels where each pixel is of size $100\times 100 \ nm^2$. In total, among all the simulated images there are $81049$ molecules. We localize the molecules on a $256\times 256$ pixel image, where the size of each pixel is $25\times 25\ nm^2$. The standard deviation of the Gaussian PSF is $\sigma=109.70\ nm$.

The average number of molecules for each acquisition is 217.

The final image of the sample has 4199 activated molecules. 

\begin{table}[H]
\centering
\begin{tabular}{l|l|l|l|l|l|l|}
\cline{2-7}
                                & $J_0$ & $J_2$ & $J_4$ & CD  & FN & FP   \\ \hline
\multicolumn{1}{|l|}{CEL0}      & 0.0424   & 0.4667   & 0.5523   & 121 & 96 & \textbf{3}    \\ \hline
\multicolumn{1}{|l|}{WCEL0}     & \textbf{0.0567}   & \textbf{0.5523}   & \textbf{0.6593}   & 151 & 67 & 14   \\ \hline
\multicolumn{1}{|l|}{DeepStorm} & 0.0247   & 0.0373   & 0.0384   & \textbf{217} & \textbf{1}  & 8157 \\ \hline
\end{tabular}
\caption{Jaccard index for $\delta=0,\ 2,\ 4$ and CD, FN, FP for $\delta=4$ computed as mean over the frames.}
\label{tabella_frame}
\end{table}


\begin{table}[H]
\centering
\begin{tabular}{l|l|l|l|l|l|l|}
\cline{2-7}
                                & $J_0$  & $J_2$  & $J_4$  & CD   & FN & FP   \\ \hline
\multicolumn{1}{|l|}{CEL0}      & 0.4201 & 0.4541 & 0.4546 & \textbf{4199} & \textbf{0}  & 5038 \\ \hline
\multicolumn{1}{|l|}{WCEL0}     & \textbf{0.4678} & \textbf{0.5665} & \textbf{0.5737} & 4198 & 1  & \textbf{3118} \\ \hline
\multicolumn{1}{|l|}{DeepStorm} & 0.3724 & 0.3743 & 0.3743 & \textbf{4199} & \textbf{0}  & 7020 \\ \hline
\end{tabular}
\caption{Jaccard index for $\delta=0,\ 2,\ 4$ and CD, FN, FP for $\delta=4$ computed on the final image.}
\end{table}

==> ISBI/overpic_prove.tex <==
\begin{overpic}[width=0.4\textwidth]{ISBI/gt.png}%
\put(50,800){\color{white}zoom}%
\put(120,700){\linethickness{0.25mm}\color{white}\line(1,-2){150}}%
\put(200,100){\linethickness{0.25mm}\color{white}\polygon(0,0)(250,0)(250,250)(0,250)}%
\end{overpic}

\begin{overpic}[width=0.25\textwidth]{ISBI/RecP.png}%
\put(1100,-150){\frame{\includegraphics[width=0.1\textwidth]{ISBI/RecP_zoom.png}}}%
\put(550,200){\linethickness{0.25mm}\color{white}\line(2.5,-1){350}}%
\put(230,110){\linethickness{0.25mm}\color{white}\polygon(0,0)(200,0)(200,200)(0,200)}%
\end{overpic}%

==> ISBI/zoom_tikz.tex <==
% \begin{ISBIure}[H]
% 	\centering
% 	\begin{tikzpicture}
	
% 	\begin{scope}[spy using outlines={rectangle,black,magnification=5,size=2.5cm}]
% 	\node {	\includegraphics[height=2.5cm]{ISBI/Acq.png}};
% 	\spy on (-0.45,-0.45) in node [name=c1]  at (0,0);
% 	\end{scope}
% 	\node[below of=c1, align=center, node distance=1.4cm] {\scalebox{1}{$\overline{\mathbf{y}}$}};
	
% 	\begin{scope}[spy using outlines={rectangle,black,magnification=5,size=2.5cm}]
% 	\node {	\includegraphics[height=2.5cm]{ISBI/RecG.png}};
% 	\spy on (-0.45,-0.45) in node [name=c2]  at (2.1,0);
% 	\end{scope}
% 	\node[below of=c2, align=center, node distance=1.4cm] {\scalebox{1}{CEL0}};
	
% 	\begin{scope}[spy using outlines={rectangle,black,magnification=5,size=2.5cm}]
% 	\node {	\includegraphics[height=2.5cm]{ISBI/RecP.png}};
% 	\spy on (-0.45,-0.45) in node [name=c3]  at (4.2,0);
% 	\end{scope}
% 	\node[below of=c3, align=center, node distance=1.4cm] {\scalebox{1}{wCEL0}};
	
% 	\begin{scope}[spy using outlines={rectangle,black,magnification=5,size=2.5cm}]
% 	\node {	\includegraphics[height=2.5cm]{ISBI/Rec_deepstorm.png}};
% 	\spy on (-0.45,-0.45) in node [name=c4]  at (6.3,0);
% 	\end{scope}
% 	\node[below of=c4, align=center, node distance=1.4cm] {\scalebox{1}{Deep-STORM}};
	
% 	\end{tikzpicture}
	
% 	\caption{Close-up on a detail of the reconstructions with CEL0, WCEL0 and DeepStorm in comparison with the acquisition.}
% 	\label{ISBI:close-ups}

% \end{ISBIure}


\begin{ISBIure}[H]
	\centering
	\begin{tikzpicture}
	
	\begin{scope}[spy using outlines={rectangle,black,magnification=5,size=2.5cm}]
	\node {	\includegraphics[height=2.5cm]{ISBI/RecG.png}};
	\spy on (-0.45,-0.45) in node [name=c2]  at (0,0);
	\end{scope}
	\node[below of=c2, align=center, node distance=1.4cm] {\scalebox{1}{CEL0}};
	
	\begin{scope}[spy using outlines={rectangle,black,magnification=5,size=2.5cm}]
	\node {	\includegraphics[height=2.5cm]{ISBI/RecP.png}};
	\spy on (-0.45,-0.45) in node [name=c3]  at (2.7,0);
	\end{scope}
	\node[below of=c3, align=center, node distance=1.4cm] {\scalebox{1}{wCEL0}};
	
	\begin{scope}[spy using outlines={rectangle,black,magnification=5,size=2.5cm}]
	\node {	\includegraphics[height=2.5cm]{ISBI/Rec_deepstorm.png}};
	\spy on (-0.45,-0.45) in node [name=c4]  at (5.4,0);
	\end{scope}
	\node[below of=c4, align=center, node distance=1.4cm] {\scalebox{1}{Deep-STORM}};
	
	\end{tikzpicture}
	
	\caption{Close-up on a detail of the reconstructions with CEL0, WCEL0 and DeepStorm in comparison with the acquisition.}
	\label{ISBI:close-ups}

\end{ISBIure}

==> fig.tex <==
% 2x3 con gt, acq, frame acq e le tre ricostruzioni a confronto
\begin{figure}[h!]    
\centering
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/gt}
\caption{GT}
\label{fig:gt}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/Acq}
\caption{$\overline{\mathbf{y}}$}
\label{fig:data}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/Acqframe.png}
\caption{Single frame}
\label{fig:frame}
\end{subfigure} \\
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/RecP}
\caption{wCEL0}
\label{fig:wCEL0}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/RecG}
\caption{CEL0}
\label{fig:CEL0}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/Rec_deepstorm.png}
\caption{Deep-STORM}
\label{fig:DS}
\end{subfigure}
 \caption{Results for the ISBI SMLM 2013 dataset. First row: (a) Ground Truth data, (b) sum of all acquisitions (x4), (c) single acquisition (x4), (d) wCEL0 result, (e) CEL0 result, (f) Deep-STORM result.}
    \label{fig:my_label}
\end{figure}

%1x4 zoom con acq e tre ricostruzioni
\begin{figure}[h!]    
\begin{subfigure}[b]{0.115\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/Acq_zoom.png}
\caption{$\overline{\mathbf{y}}$}
\label{fig:data_zoom}
\end{subfigure}
\begin{subfigure}[b]{0.115\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/RecP_zoom.png}
\caption{wCEL0}
\label{fig:wCEL0_zoom}
\end{subfigure}
\begin{subfigure}[b]{0.115\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/RecG_zoom.png}
\caption{CEL0}
\label{fig:CEL0_zoom}
\end{subfigure}
\begin{subfigure}[b]{0.115\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/Rec_deepstorm_zoom.png}
\caption{Deep-Storm}
\label{fig:DS_zoom}
\end{subfigure}
\caption{Close-ups: (a) sum of all acquisitions, (b) wCEL0 result, (c) CEL0 result, (d) Deep-STORM result.}
    \label{fig:close-ups}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1x3 gt, acq e acq di un frame
\begin{figure}[h!]    
\centering
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/gt}
\caption{GT}
\label{fig:gt}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/Acq}
\caption{$\overline{\mathbf{y}}$}
\label{fig:data}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ISBI/Acqframe.png}
\caption{Single frame}
\label{fig:frame}
\end{subfigure} 
 \caption{ISBI SMLM 2013 dataset: (a) Ground Truth data, (b) sum of all acquisitions (x4), (c) single acquisition (x4)}
    \label{fig:my_label}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% overpic ricostruzioni
\begin{figure}[h!]    
\centering
\begin{subfigure}[b]{0.15\textwidth}
\centering
\begin{overpic}[width=\textwidth]{ISBI/RecP.png}%
\put(230,110){\linethickness{0.25mm}\color{white}\polygon(0,0)(200,0)(200,200)(0,200)}%
\end{overpic}%
\caption{wCEL0}
\label{fig:wCEL0}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\begin{overpic}[width=\textwidth]{ISBI/RecG.png}%
\put(230,110){\linethickness{0.25mm}\color{white}\polygon(0,0)(200,0)(200,200)(0,200)}%
\end{overpic}%
\caption{CEL0}
\label{fig:CEL0}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\begin{overpic}[width=\textwidth]{ISBI/Rec_deepstorm.png}%
\put(230,110){\linethickness{0.25mm}\color{white}\polygon(0,0)(200,0)(200,200)(0,200)}%
\end{overpic}%
\caption{Deep-STORM}
\label{fig:DS}
\end{subfigure}\\
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{ISBI/RecP_zoom.png}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{ISBI/RecG_zoom.png}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{ISBI/Rec_deepstorm_zoom.png}
\end{subfigure}
\caption{(a) wCEL0 result, (b) CEL0 result, (c) Deep-STORM result.}
\label{fig:close-ups}
\end{figure}

